Neural Discourse Structure for Text Categorization

We show that discourse structure, as defined by Rhetorical Structure Theory and provided by an existing discourse parser, benefits text categorization. Our approach uses a recursive neural network and a newly proposed attention mechanism to compute a representation of the text that focuses on salient content, from the perspective of both RST and the task. Experiments consider variants of the approach and illustrate its strengths and weaknesses.

==> discussion.tex <==
\section{Discussion}
\label{sec:discussion}

==> figures/model.tex <==
% In the preamble:


% In the document:
\begin{dependency}[theme = simple]
   \begin{deptext}[column sep=1em]
      \unit{1} \& \unit{2} \& \unit{3} \& \unit{4} \& \unit{5} \& \unit{6} \& \unit{7} \& \unit{8} \\
   \end{deptext}
   \deproot{8}{ROOT}
   \depedge{1}{8}{Concession}
   \depedge{2}{1}{Justify}
   \depedge{4}{1}{Justify}
   \depedge{5}{1}{Justify}
   \depedge{3}{2}{Elaboration}
   \depedge{6}{5}{Justify}
   \depedge{7}{5}{Justify}
\end{dependency}

\unittext{It could have been a great movie.}{1}
\unittext{It does have beautiful scenery,}{2}
\unittext{some of the best since Lord of the Rights.}{3}
\unittext{The acting is well done,}{4}
\unittext{and I really liked the son of the leader of the Samurai.}{5}
\unittext{He was a likable chap,}{6}
\unittext{and I hated to see him die.}{7}
\unittext{But, other than all that, this movie is nothing more than hidden rip-offs}{8}

==> rstparser.tex <==
\section{More details about the RST Parser}
\label{append:rstparser}

==> task-frame.tex <==
\section{Task II: Frame Prediction}
\label{sec:frame}

% ----------------------------------------
\subsection{Data}
\label{subsec:frame-data}

The Media Frames Corpus \cite[MFC]{} consists of annotations for approximately 4,200 articles about immigration taken from 13 U.S. news- papers over the years 1980–2012. The annotations for these articles are in terms of a set of 15 general purpose “framing dimensions” (such as Politics and Legality), developed to be broadly applicable to a variety of issues, and to be recognizable in text (by trained annotators). Each article has been annotated with a “primary frame” (the overall dominant aspect of immigration being emphasized), as well as an overall “tone” (pro, neutral, or anti), which is the extent to which a pro-immigration advocate would like to see the article in print, without implying any any stance taken by the author.2 The MFC contains at least two independent annotations for each article; agreement on the primary frame and tone was established through discussion in cases of initial disagreement. A complete list of these framing dimensions is given in the supplementary material.

% ----------------------------------------
\subsection{Data Processing}
\label{subsec:frame-processing}



==> task-sentiment.tex <==
\section{Task I: Document-level Sentiment Analysis}
\label{sec:sentiment}

\subsection{Task Description}
\label{subsec:sentiment-task}

\begin{itemize}
\item task description
\item data
\item label
\end{itemize}

\subsection{Data Processing}
\label{subsec:sentiment-processing}

\begin{itemize}
\item 
\end{itemize}

==> task-vote.tex <==
\section{Task III: Congress Vote Prediction}
\label{sec:vote}
